Sample-Optimal Density Estimation in Nearly-Linear Time

We design a new, fast algorithm for agnostically learning univariate probability distributions whose densities are well approximated by piecewise polynomial functions. Let $f$ be the density function of an arbitrary univariate distribution, and suppose that $f$ is $\mathrm{OPT}$-close in $L_1$-distance to an unknown piecewise polynomial function with $t$ interval pieces and degree $d$. Our algorithm draws $n = O(t(d+1)/\epsilon^2)$ samples from $f$, runs in time $\tilde{O}(n \cdot \mathrm{poly}(d))$, and with probability at least $9/10$ outputs an $O(t)$-piecewise degree-$d$ hypothesis $h$ that is $4 \cdot \mathrm{OPT} +\epsilon$ close to $f$. Our general algorithm yields (nearly) sample-optimal and nearly-linear time estimators for a wide range of structured distribution families over both continuous and discrete domains in a unified way. For most of our applications, these are the first sample-optimal and nearly-linear time estimators in the literature. As a consequence, our work resolves the sample and computational complexities of a broad class of inference tasks via a single "meta-algorithm". Moreover, we experimentally demonstrate that our algorithm performs very well in practice. Our algorithm consists of three "levels": (i) At the top level, we employ an iterative greedy algorithm for finding a good partition of the real line into the pieces of a piecewise polynomial. (ii) For each piece, we show that the sub-problem of finding a good polynomial fit on the current interval can be solved efficiently with a separation oracle method. (iii) We reduce the task of finding a separating hyperplane to a combinatorial problem and give an efficient algorithm for this problem. Combining these three procedures gives a density estimation algorithm with the claimed guarantees.

==> polys.tex <==
\section{Properties of polynomials}
\label{sec:polys}
Before we construct our fast $\Ak$-projection oracle for the class of
non-negative polynomials, we introduce auxiliary results for
polynomials with a fixed degree $\pdeg$. 

\subsection{Bounds on coefficients of bounded polynomials}
We first bound the absolute value of the coefficients of polynomials
with bounded norms of their integrals. This will be useful when we
analyze the running time of our algorithm. In particular:
\begin{lemma}
\label{lem:polybound2}
Let $p_c$ be a degree-\pdeg{} polynomial with coefficients $c \in \R^{m+1}$ such that $p(x) \geq 0$ for $x \in [-1, 1]$ and $\int_{-1}^1 p(x) \diff x \leq \alpha$, where $\alpha > 0$, for some $0 < k \leq \pdeg$.
Then we have
\[
  \abs{c_i} \leq \alpha \cdot (m + 1)^2 \cdot (\sqrt{2} + 1)^m \quad \text{for all } i = 0, \ldots, m \; .
\]
\end{lemma}
This lemma is proved in Section~\ref{app:markov-proof}.

\subsection{Testing non-negativity of polynomials}
\label{sec:non-neg-poly}
In addition to the structural results introduced above, we also need a procedure for checking whether a given polynomial is non-negative on a given interval.
We later use this procedure to ensure that we only produce non-negative density estimates.
Unfortunately, we have to allow for a certain amount of noise in our problem statement because we cannot find roots of polynomials exactly.
Formally, the testing problem we solve is the following:

\begin{definition}[Approximate non-negativity test]
\label{prob:nonneg}
An approximate non-negativity tester is an algorithm satisfying the following guarantee.
Given a polynomial $p = \sum_{i = 0}^m c_i x^i$ with $\max_i \abs{c_i} \leq \alpha$ and a parameter $\mu > 0$, return one of two results:
\begin{itemize}
\item a point $x \in [-1, 1]$ at which $p(x) < -\mu / 2$ if there exists a point $x' \in [-1, 1]$ so that $p(x') < -\mu$.
\item ``OK'' otherwise.
\end{itemize}
\end{definition}

The following theorem now gives an approximate non-negativity tester.
\begin{theorem}
Consider $p$ and $\mu$ from Definition~\ref{prob:nonneg}.
Then there exists an algorithm \textsc{Test-Nonneg}$(p, \mu)$ that is an approximate non-negativity tester and runs in time
\[
  O(m \log^2 m \cdot (\log^2 m + \log \log \alpha + \log \log (1 / \mu))) \; ,
\]
where $\alpha$ is the bound on the coefficients of $p$.
\end{theorem}

This result is proved in Section~\ref{app-non-neg}. 

